Cooperative Learning for Cost-Adaptive Inference

We propose a cooperative training framework for deep neural network architectures that enables the runtime network depths to change to satisfy dynamic computing resource requirements. In our framework, the number of layers participating in computation can be chosen dynamically to meet performance-cost trade-offs at inference runtime. Our method trains two Teammate nets and a Leader net, and two sets of Teammate sub-networks with various depths through knowledge distillation. The Teammate nets derive sub-networks and transfer knowledge to them, and to each other, while the Leader net guides Teammate nets to ensure accuracy. The approach trains the framework atomically at once instead of individually training various sizes of models; in a sense, the various-sized networks are all trained at once, in a "package deal." The proposed framework is not tied to any specific architecture but can incorporate any existing models/architectures, therefore it can maintain stable results and is insensitive to the size of a dataset's feature map. Compared with other related approaches, it provides comparable accuracy to its full network while various sizes of models are available.

==> draw/arch_adaptive_net.tex <==
%\begin{figure}[t]
%  \centering
%  \includegraphics[, width=0.4\textwidth]{draw/pics/arch_adaptive_net.pdf}
%  \caption{Deriving sub-networks.}
%\label{fig:arch_adaptive_net}
%\end{figure}
\begin{wrapfigure}{r}{0.43\textwidth}
  \hspace{-1.0cm}
  \begin{center}
    \includegraphics[, width=0.43\textwidth]{draw/pics/arch_adaptive_net.pdf}
  \end{center}
  \caption{Deriving sub-networks.}
  \label{fig:arch_adaptive_net}
\end{wrapfigure}

==> draw/mask.tex <==
\begin{figure}[t]
\centering 
\includegraphics[width=0.67\linewidth]{draw/pics/mask.pdf}
\caption{Masking: selecting layers from neural networks with residual connections by the global mask.}
\todo[inline]{Please incorporate some/all of the equations (14)-(17) in Fig 4}
\label{fig:mask}
\end{figure}

==> draw/method.tex <==
%\begin{figure}[t]
%\centering 
%\includegraphics[width=0.5\linewidth]{draw/pics/method.pdf}
%\caption{The entire Cooperative training framework.}
%\label{fig:method}
%\end{figure}
\begin{wrapfigure}{r}{0.42\textwidth}
  \hspace{-2.5cm}
  \begin{center}
    \includegraphics[width=0.42\textwidth]{draw/pics/method.pdf}
  \end{center}
  \caption{The entire Cooperative training framework.}
  \label{fig:method}
\end{wrapfigure}

==> draw/overview.tex <==
\begin{figure}[t]
\centering 
\subfigure[Typical]{
\label{fig:overview_1}
\includegraphics[width=0.23\linewidth]{draw/pics/typical_knowledge_distillation.pdf}}
\subfigure[Mutual]{
\label{fig:overview_2}
\includegraphics[width=0.23\linewidth]{draw/pics/mutual_knowledge_distillation.pdf}}
\subfigure[Self (\emph{a.k.a} inplace)]{
\label{fig:overview_3}
\includegraphics[width=0.23\linewidth]{draw/pics/self_knowledge_distillation.pdf}}
\subfigure[Ours]{
\label{fig:overview_4}
\includegraphics[width=0.22\linewidth]{draw/pics/team-cooperative_self_knowledge_distillation.pdf}}
\caption{Overview of different knowledge distillations. (d) is enlarged in Fig.~\ref{fig:method}.}
\label{Fig: overview}
\end{figure}

==> figs/fig_ablation_scaling_factor.tex <==
\begin{figure}[H]
\centering 
\includegraphics[width=0.7\linewidth]{figs/pics/ablation_scaling_factor.png}
\caption{.}
\label{Fig:ablation_scaling_factor}
\end{figure}

==> figs/fig_ablation_sfsl.tex <==
\begin{figure}[H]
\centering 
\includegraphics[width=0.7\linewidth]{figs/pics/ablation_sfsl.png}
\caption{Accuracy on CIFAR-100 in different models with or without Scaling Factor Sensitive Loss}
\label{Fig:ablation_scaling_factor_sensitive_loss}
\end{figure}

==> figs/fig_cifar100_acc_flop.tex <==
\begin{figure*}[t]
\centering 
\subfigure[Acc. and FLOPs]{
\label{Fig: cifar100_acc_flop_sub1}
\includegraphics[width=0.25\linewidth]{figs/pics/cifar100_acc_flops.png}
}
\subfigure[Acc. and \#Parameters]{
\label{Fig: cifar100_acc_flop_sub2}
\includegraphics[width=0.25\linewidth]{figs/pics/cifar100_acc_para.png}
}
\subfigure[Acc. and Time of Inference]{
\label{Fig: cifar100_acc_flop_sub3}
\includegraphics[width=0.25\linewidth]{figs/pics/cifar100_acc_flops.png}
}
\\
\subfigure[Acc. and FLOPs]{
\label{Fig: cifar100_acc_flop_sub1}
\includegraphics[width=0.25\linewidth]{figs/pics/cifar100_acc_flops.png}
}
\subfigure[Acc. and \#Parameters]{
\label{Fig: cifar100_acc_flop_sub2}
\includegraphics[width=0.25\linewidth]{figs/pics/cifar100_acc_para.png}
}
\subfigure[Acc. and Time of Inference]{
\label{Fig: cifar100_acc_flop_sub3}
\includegraphics[width=0.25\linewidth]{figs/pics/cifar100_acc_flops.png}
}
\caption{Performance and costs of different methods on CIFAR100 (first row) and Tiny ImageNet (second row)}
\label{Fig: cifar100_acc_flop}
\end{figure*}

==> figs/fig_example.tex <==
\begin{figure}[H]
\centering 
\subfigure[name1]{
\label{Fig.sub.1}
\includegraphics[width=0.45\linewidth]{figs/pics/fig_example.png}}
\subfigure[name2]{
\label{Fig.sub.2}
\includegraphics[width=0.45\linewidth]{figs/pics/ablation.png}}
\caption{Example figure \ref{Fig.main} has two sub figures, fig. \ref{Fig.sub.1} is the travel demand of driving auto, and fig. \ref{Fig.sub.2} is the travel demand of park-and-ride.}
\label{Fig.main}
\end{figure}

==> tables/tab_abaltion_description.tex <==
\begin{table}[ht]
  \caption{Description of networks' configurations}
  
  \label{tab:ablation_every_component_settings}
  
  \centering
  \resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{lclllll}
    \toprule
    Network Name& Random Sampling Mid  &  Configuration           &  Scaling Ratios \\
    \midrule
    LS-Net      & \XSolidBrush         &  $1 max + 2 mid + 1 min$  &  $[1.0, 0.7, 0.4, 0.2]$     \\
    ULS-Net     & \Checkmark           &  $1 max + 2 mid + 1 min$  &  $[1.0, \mathcal{?}, ?, 0.2]$     \\
    MLS-Net     & \XSolidBrush         &  $(1 max + 2 mid + 1 min) \times 2$  &  $[1.0, 0.7, 0.4, 0.2]$     \\
    UMLS-Net    & \Checkmark         &  $(1 max + 2 mid + 1 min) \times 2$  &  $[1.0, 0.7, 0.4, 0.2]$     \\
    TCLS-Net    & \XSolidBrush         &  $(1 max + 2 mid + 1 min) \times 2 + 1 max$  &  $[1.0, 0.7, 0.4, 0.2]$     \\
    UTCLS-Net   & \Checkmark           &  $(1 max + 2 mid + 1 min) \times 2 + 1 max$  &  $[1.0, ?, ?, 0.2]$     \\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/tab_ablation_scaling_factors.tex <==
\begin{table}[ht]
  \caption{Networks' configurations of intermediate scaling factors setting strategies}
  \label{tab:random_and_fixed}
  \centering
  \resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{lccc}
    \toprule
    Network Name    & Random Sampling Mid  &  Configuration            &  Ratios \\
    \midrule
    LS-ResNet152    & \XSolidBrush         &  $1 max + 2 mid + 1 min$  &  $[1.0, 0.7, 0.4, 0.2]$     \\
    ULS-ResNet152   & \Checkmark           &  $1 max + 2 mid + 1 min$  &  $[1.0, \mathcal{?}, ?, 0.2]$     \\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/tab_cifar100.tex <==
\begin{table}[ht]
  \caption{Networks' performance on CIFAR-100.}
  \label{tab:cifar100}
  
  \centering
  \resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{lcccc}
    \toprule
    Network        &  Execution Part & \#Parameters &  FLOPs  &  Acc.($\%$)         \\
    \midrule
    \multirow{4}{*}{B-ResNet152}    
                    &                 &            &         &                     \\
                    &                 &            &         &                     \\
                    &                 &            &         &                     \\
                    &                 &            &         &                     \\
    \midrule
    \multirow{4}{*}{BYOT-ResNet152}    
                    &                 &            &         &                     \\
                    &                 &            &         &                     \\
                    &                 &            &         &                     \\
                    &                 &            &         &                     \\
    \midrule
    LS-ResNet152   &                 &            &         &                     \\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/tab_exp_abalation_sfsl.tex <==
\begin{table}[ht]
  \caption{Comparison between fixed and random intermediate depth.}
  \label{tab:ablation_sfst}
  
  \centering
  \resizebox{.9\columnwidth}{!}{
  \begin{tabular}{ccc}
    \toprule
                    & \multicolumn{2}{c}{Acc.(\%)}  \\
    \cmidrule(lr){2-3}
    Scaling Ratio   &  LS-ResNet152 w/ SFSL & ULS-ResNet152 w/ SFSL     \\
    \midrule
            1.0     &       74.61   &   73.59\\
            0.8     &       75.17   &   75.52\\
            0.6     &       75.70   &   76.33\\
            0.4     &       76.55   &   75.85\\
            0.2     &       72.09   &   70.89\\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/tab_exp_ablation_every.tex <==
\begin{table}[ht]
  \caption{Performance comparison (accuracy) of different methods for}
  \label{tab:exp_ablation_every}
  \centering
  \resizebox{.85\columnwidth}{!}{
  \begin{tabular}{lccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{5}{c}{Acc.(\%)} \\
    \cmidrule(r){2-6}
    Network    & $0.2\times$ & $0.4\times$ & $0.6\times$ & $0.8\times$ & $1.0\times$ \\
    \midrule
    LS-Net     &             &             &             &             &      \\
    ULS-Net    &             &             &             &             &      \\
    MLS-Net    &             &             &             &             &      \\
    MLS-Net    &             &             &             &             &      \\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/tab_exp_ablation_random.tex <==
\begin{table}[ht]
  \caption{Comparison of the two different training approaches, with fixed and random intermediate depth.}
  \label{tab:ablation_random}
  \centering
  \resizebox{.7\columnwidth}{!}{
  \begin{tabular}{ccc}
    \toprule
                    & \multicolumn{2}{c}{Acc.(\%)}  \\
    \cmidrule(lr){2-3}
    Scaling Ratio   &  \textsf{LS}-ResNet152 & \textsf{ULS}-ResNet152       \\
    \midrule
            1.0     &       62.99   &   74.40\\
            0.8     &       68.02   &   73.66\\
            0.6     &       70.02   &   74.05\\
            0.4     &       69.37   &   71.52\\
            0.2     &       62.04   &   65.44\\
    \bottomrule
  \end{tabular}
  }
\end{table}

==> tables/tab_exp_cifar100.tex <==
\begin{table}[ht]
  \caption{Performance comparison (accuracy) of different methods for}
  \label{sample-table}
  \centering
  \begin{tabular}{lccccc}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{5}{c}{Sub-Net Ratio} \\
    \cmidrule(r){2-6}
    Network    & $0.2\times$ & $0.4\times$ & $0.6\times$ & $0.8\times$ & $1.0\times$ \\
    \midrule
    LS-Net     &             &             &             &             &      \\
    ULS-Net    &             &             &             &             &      \\
    MLS-Net  w/o sub-net learning    &             &             &             &             &      \\
    MLS-Net    &             &             &             &             &      \\
    \bottomrule
  \end{tabular}
\end{table}

==> tables/tab_tinyimagenet.tex <==
\begin{table}[ht]
  \caption{Networks' performance on tiny ImageNet.}
  \label{tab:tiny_imagenet}
  
  \centering
  \resizebox{1.0\columnwidth}{!}{
  \begin{tabular}{lcccc}
    \toprule
    Network        &  Execution Part & \#Parameters &  FLOPs  &  Acc.($\%$)         \\
    \midrule
    \multirow{1}{*}{Baseline-ResNet152}    
        &   all             &            &         &                    \\
    \midrule
    \multirow{4}{*}{B-ResNet152}    
        &   $1^{st}$ exit   &            &         &    42.05                 \\
        &   $2^{nd}$ exit   &            &         &    48.25                 \\
        &   $3^{rd}$ exit   &            &         &    57.46                 \\
        &   $4^{th}$ exit   &            &         &    60.35                 \\
    \midrule
    \multirow{4}{*}{BYOT-ResNet152}    
        &   $1^{st}$ exit   &            &         &    24.62
              ^  \\
        &   $2^{nd}$ exit   &            &         &    52.05
              ^  \\
        &   $3^{rd}$ exit   &            &         &    64.57
              ^  \\
        &   $4^{th}$ exit   &            &         &    64.01
                 \\
    \midrule
    LS-ResNet152   &                 &            &         &                     \\
    \bottomrule
  \end{tabular}
  }
\end{table}
